Explaining Predictions from Machine Learning Models: Algorithms, Users, and Pedagogy

Model explainability has become an important problem in machine learning (ML) due to the increased effect that algorithmic predictions have on humans. Explanations can help users understand not only why ML models make certain predictions, but also how these predictions can be changed. In this thesis, we examine the explainability of ML models from three vantage points: algorithms, users, and pedagogy, and contribute several novel solutions to the explainability problem.

==> 02-background/main.tex <==
% !TEX root = ../thesis-main.tex

\chapter{Background}
\label{chapter:background}

\footnote[]{This chapter was published as~\citep{...}.}
\acresetall

Prior to 2018, all theses had a related work chapter, followed by chapters corresponding to three or more published papers.

From 2018 onwards, a thesis may also do without related work chapter, and it needs to have four chapters based on four or more published papers.  

The related work chapter. Usually just a collection of the related work sections of the papers, with some additional introducing background work on your area (e.g., introduction to IR). List here which topics you discuss in this section.

Of course, you could refer to the work by \citet{meij2010thesis} or \citet{weerkamp2011thesis}.

==> 03-methodology/main.tex <==
% !TEX root = thesis-main.tex

\chapter{Methodology}
\label{chapter:methodology}

\footnote[]{This chapter was published as~\citep{...}.}
\acresetall

A chapter on the general research methodology. You can use this chapter to introduce your baseline system, if it is the same in several chapters (e.g., language modeling). Also, you can list the document collections you use here (e.g., TREC collections, with details of the collection, topics, assessments, preprocessing, etc.). Finally, introduce metrics you refer to in research chapters and explain why you use these, and give details on significance tests you use.

Just put everything in here that is used in more than one research chapter, you can simply refer back to this chapter.

==> 04-research-pedagogy/sections/abstract.tex <==
%!TEX root = ../main.tex

In this work, we explain the setup for a technical, graduate-level course on Fairness, Accountability, Confidentiality, and Transparency in Artificial Intelligence (FACT-AI) at \OurUniversity{}, which teaches FACT-AI concepts through the lens of reproducibility. 
The focal point of the course is a group project based on reproducing existing FACT-AI algorithms from top AI conferences and writing a corresponding report. 
In the first iteration of the course, we created an open source repository with the code implementations from the group projects. 
In the second iteration, we encouraged students to submit their group projects to the Machine Learning Reproducibility Challenge, resulting in 9 reports from our course being accepted for publication in the ReScience journal. 
We reflect on our experience teaching the course over two years, where one year coincided with a global pandemic, and propose guidelines for teaching FACT-AI through reproducibility in graduate-level AI study programs. 
We hope this can be a useful resource for instructors who want to set up similar courses in the future. 

==> 04-research-pedagogy/tables/feedback.tex <==
\begin{table}[h]
\caption{Feedback about the course.}
\centering
\begin{tabular}{@{}l@{}}
\toprule
(a) Feedback from students \\
\midrule
\begin{minipage}[t]{\columnwidth}
\begin{itemize}[leftmargin=*]
    \item ``Reproducing an article was hard and intensive but a really good experience.''
     \item ``Replicating another study, seeing how (poorly) other research is performed was really eye-opening.''
    \item ``Reproducing a paper: I believe this is a good thing to do and is an important part of academia.''
    \item  ``Gave good insights into the trustworthiness of research papers, which is apparently not great.''
    \item ``I appreciate the critical view I have developed on papers as a result of this course. Normally I would easily accept the content of a paper, but I will be more critical from now on, as many papers are not reproducible.''
    \item ``I think it's really good that we get some practical insights into reproducing results from other papers, not all papers are as good as they seem to be.''
    \item ``I really appreciated that this was the first course where students are judging state-of-the-art AI-models. In other words, students were able to experience the scientific workfield of AI.''
\end{itemize}
\end{minipage}
\\ \\
\midrule
(b) Feedback from the ML Reproducibility Challenge \\
\midrule
\begin{minipage}[t]{\columnwidth}
\begin{itemize}[leftmargin=*]
\item ``The report reveals a lot of dark spots of the original paper.''
\item ``Good reviews, strong reproducibility report, provides code reimplementation from scratch which is a strong contribution.''
\item ``The discussion section is a great reference point for future work.''
\item ``The additional experimentation is rather impressive and the report reflects  an intuitive understanding of concepts such as  coverage, correctness, and counterfactual explanations.''
\item ``The report provides good insights on how the experiments in the original paper actually work, while also generating new hypothesis to be tested for future research, which is a positive outcome.''
\item ``My main concern is that it remains unclear why some of the results are so far off from the original paper? I would have expected the authors to dig deeper on that.''
%\item ``The paper is generally difficult to follow. The paper reads closer to an outline than a finished report.''
\item ``It doesn't go above and beyond the reproduction and does not offer novel insights into the workings of the original paper.''
\item ``The submission failed at reproducing the original results. It is unclear whether this is due to a difference in the experimental setup or due to implementation errors. ''
%\item ``The paper reads closer to an outline than a finished report. I would encourage the authors to spend some additional time on organization, making sure that the key takeaways are made plain and that the report reads fluidly throughout.''
\end{itemize}
\end{minipage}
\end{tabular}
\label{tab:feedback}
\end{table}
